XAMBA: Enabling Efficient State Space Models on Resource-Constrained Neural Processing Units

State-Space Models (SSMs) have emerged as efficient alternatives to transformers for sequential data tasks, offering linear or near-linear scalability with sequence length, making them ideal for long-sequence applications in NLP, vision, and edge AI, including real-time transcription, translation, and contextual search. These applications require lightweight, high-performance models for deployment on resource-constrained devices like laptops and PCs. Designing specialized accelerators for every emerging neural network is costly and impractical; instead, optimizing models for existing NPUs in AI PCs provides a scalable solution. To this end, we propose XAMBA, the first framework to enable and optimize SSMs on commercial off-the-shelf (COTS) state-of-the-art (SOTA) NPUs. XAMBA follows a three-step methodology: (1) enabling SSMs on NPUs, (2) optimizing performance to meet KPI requirements, and (3) trading accuracy for additional performance gains. After enabling SSMs on NPUs, XAMBA mitigates key bottlenecks using CumBA and ReduBA, replacing sequential CumSum and ReduceSum operations with matrix-based computations, significantly improving execution speed and memory efficiency. Additionally, ActiBA enhances performance by approximating expensive activation functions (e.g., Swish, Softplus) using piecewise linear mappings, reducing latency with minimal accuracy loss. Evaluations on an Intel Core Ultra Series 2 AI PC show that XAMBA achieves up to 4.8X speed-up over the baseline. Our implementation is available at https://github.com/arghadippurdue/XAMBA.

==> 2_motivation.tex <==
\section{Motivation} \label{sec_motivation}


While SSMs provide notable efficiency advantages, deploying them on NPUs presents unique challenges due to their computational patterns and hardware requirements. Unlike traditional deep learning models, SSMs exhibit characteristics that deviate from standard kernel operations, necessitating specialized optimizations. Existing NPUs are designed primarily for data-parallel operations like matrix multiplications, which dominate workloads in transformers and CNNs. SSMs, however, involve sequential computations and specialized operators, such as activation functions (e.g., Swish and Softplus) and cumulative summations (CumSum). These operations do not align with the highly parallelized architecture of NPUs, leading to inefficient execution when mapped directly. Fig.~\ref{fig:motivation_exec_lat_brkdwn} highlights execution bottlenecks for Mamba and Mamba-2 models on the Intel\textregistered\ Core\texttrademark\ Ultra Series 2~\cite{lnl} NPU. For Mamba, the majority of execution time is consumed by activation functions, such as Swish (SiLU) and Softplus, which are executed sequentially on DSPs. These DSPs are less optimized for such operations, resulting in prolonged execution times and underutilization of the data-parallel units. In Mamba-2, CumSum and ReduceSum emerge as primary bottlenecks, as these operations also rely on DSPs for sequential processing. This sequential nature hinders efficient reuse of local SRAM, increasing memory traffic and access latency. Both models further face challenges with elementwise multiplication (Multiply), which similarly runs on DSPs and contributes to inefficiencies. Handling long sequences in SSMs requires careful memory optimization. Limited on-chip memory must be utilized effectively to avoid frequent off-chip memory accesses, which incur significant latency and energy costs. The lack of optimized dataflow alignment for SSM computations exacerbates this issue, leading to poor performance. Blind, out-of-the-box mapping of SSMs on NPUs results in suboptimal performance, leaving much of their potential benefits untapped. Addressing these challenges is essential to fully leverage the advantages of SSMs in resource-constrained environments.






==> 3_prior_art.tex <==
\section{Prior Arts}\label{sec_prior_art}
Several efforts have been made to enable and optimize State Space Models (SSMs) for execution on hardware accelerators like GPUs. These works have made progress in improving the computational efficiency of state-space models for sequence modeling. However, they face significant limitations, which are addressed by the proposed XAMBA approach. Yang et al. (2019)~\cite{ssm_gpu} presented a GPU-optimized framework for accelerating state-space models, focusing on efficiently handling sequential data by optimizing memory transfers and reducing overheads. While this work demonstrated improved throughput, it still relied on GPU-centric architectures, which are not ideal for the memory and throughput challenges of resource-constrained edge devices. Moreover, the solution did not fully explore the specific needs of SSMs in terms of memory management and sequential computation, which are crucial for NPUs. This gap is significant because NPUs are optimized for high-throughput, parallelized computation, which requires more specialized mapping techniques for sequential models like SSMs. Wang et al. (2018)~\cite{rnn_npu} explored deploying LSTM models on NPUs, proposing custom kernels and memory optimization strategies that reduce off-chip memory access and improve data locality. Their work demonstrated improvements in the execution of recurrent models on NPUs, focusing on reducing latency and optimizing memory usage. However, their focus was primarily on traditional recurrent networks (LSTMs) rather than state-space models. The sequential nature of SSMs and the unique dataflow patterns they require for efficient execution on NPUs were not fully addressed. This is a limitation because SSMs, like Mamba, require novel kernel designs and optimizations specific to their compact representations and sequential computations. Without such optimizations, NPUs cannot fully exploit the advantages of SSMs, leading to suboptimal performance. Kiamarzi et al. (2021)~\cite{ssm_fpga} proposed a systematic approach for implementing state-space models in register transfer level (RTL), with a focus on neural network implementation. Their method can be applied to linear/nonlinear and time-varying/time-invariant systems, offering a framework for hardware synthesis of state-space equations. While this approach provides a foundation for hardware implementation, it does not specifically address the unique challenges of deploying SSMs on NPUs, such as dataflow alignment and memory optimization. Additionally, the approach may not fully leverage the parallel processing capabilities of NPUs, which are crucial for achieving high performance in resource-constrained environments. Behrouz et al. (2024)~\cite{mambamixer} introduced MambaMixer, an efficient selective state-space model with dual token and channel selection. This architecture aims to enhance the performance of SSMs by selectively mixing information across tokens and channels. While MambaMixer offers improvements in model efficiency and performance, it does not specifically address the hardware optimization aspects required for efficient execution on NPUs. The integration of such models into hardware accelerators necessitates specialized kernel designs and memory management strategies to fully exploit the capabilities of NPUs. Kiamarzi et al. (2024)~\cite{marca} proposed MARCA, a reconfigurable accelerator architecture designed to address the incompatibilities between Tensor Core-based architectures and Mamba's compute patterns. MARCA introduces a reduction-alternative PE array architecture, reusable nonlinear function units, and advanced buffer management strategies to address the bottlenecks of Mamba computations. While MARCA offers significant performance and energy efficiency improvements for SSMs on high-performance hardware, it does not directly address the unique kernel optimizations and memory alignment strategies critical for NPUs. Additionally, its focus on reconfigurable architecture may introduce overheads unsuitable for resource-constrained edge devices. These limitations highlight the need for more specialized approaches for deploying SSMs on NPUs. These prior works have made valuable contributions to optimizing sequential models for hardware accelerators. However, none of them directly target the unique characteristics of SSMs, especially on NPUs. The proposed XAMBA approach addresses these limitations by introducing novel kernel mappings, optimizing dataflow for sequential computations, and applying efficient memory management techniques specifically for SSMs. By leveraging the full potential of NPUs, XAMBA achieves superior performance and energy efficiency for state-space models, addressing challenges that past work has left unresolved.

==> 4_background.tex <==
\section{Background}\label{sec_background}
\subsection{Comparative Analysis of Sequential Data Models: RNNs, Transformers, and Mamba}
Recurrent Neural Networks (RNNs) have been widely used for sequential data processing due to their ability to retain internal memory. At each time step, an RNN processes a vector alongside the hidden state of the previous time step, enabling it to capture temporal dependencies. However, RNNs struggle with complex dependencies and suffer from slow training times, limiting their scalability and efficiency~\cite{rnn_limitations}. Transformers, in contrast, use self-attention mechanisms to capture global dependencies across input sequences. While transformers excel at modeling long-range dependencies and are highly parallelizable, they suffer from quadratic scaling, making them inefficient for long sequences~\cite{transformer_limitations}. 

State-Space Models (SSMs)~\cite{mamba2} offer an alternative approach, characterized by their linear structure and associative properties. Unlike RNNs, which are nonlinear, SSMs efficiently model sequential data using linear state equations. They capture temporal dependencies using a discretized model, typically employing a Zero-Order Hold (ZOH) approach to convert continuous parameters into discrete intervals. This linearity allows SSMs to perform inference more efficiently than transformers and RNNs, especially for long sequences. Mamba~\cite{mamba}, a leading SSM-based model, provides linear-time efficiency, adaptive memory compression, and significantly faster inference—up to 5$\times$ faster than transformers. This makes Mamba particularly suitable for modern AI workloads, addressing the limitations of traditional models.

\subsection{Performance and Efficiency of Mamba Compared to Transformers}
Mamba offers significant advantages over transformer-based models in computational efficiency and task performance. It achieves higher token throughput across all batch sizes. For example, with a batch size of 16, Mamba 1.4B processes 1089 tokens/second, outperforming transformer models of similar sizes, such as Transformer 1.3B (323 tokens/second) and Transformer 6.9B (120 tokens/second)~\cite{mamba_performance}. Additionally, Mamba scales efficiently to larger batch sizes, while transformers often encounter out-of-memory (OOM) issues. 

In terms of task performance, Mamba maintains high accuracy across benchmarks. The Mamba-2.8B model achieves an average accuracy of 63.3\%, with key benchmarks including LAMBADA (69.2\%), HellaSwag (66.1\%), and PIQA (75.2\%)~\cite{mamba_benchmarks}. Mamba's efficiency stems from its avoidance of the quadratic complexity of attention mechanisms, enabling it to handle long-range dependencies with lower resource requirements. This makes Mamba ideal for low-power, latency-critical environments where energy efficiency and high throughput are essential.

\subsection{Detailed Architecture of the Mamba Block}
The Mamba block is a fundamental component of the Mamba model. It begins by processing the input sequence, which is normalized using RMS normalization to stabilize training. A skip connection bypasses the block, enabling residual learning. The normalized input undergoes transformations through projection layers and a convolutional layer, followed by the SiLU activation function to introduce non-linearity. 

At the core of the block is the selective state-space model (SSM), which operates on sequences using state equations. The state equation $h_k = A h_{k-1} + B x_k$ updates the hidden state by modeling temporal dependencies through the matrix $A$ and incorporating new input $x_k$ via matrix $B$. The output equation $y_k = C h_k$ maps the hidden state to the output using the matrix $C$, with optional augmentation by another learnable matrix $D$. The output from the selective SSM block is combined with the original input using element-wise operations, followed by another RMS normalization. Finally, the output is passed through a task-specific linear layer and a softmax function to generate predictions. This block is repeated $n$ times in the overall Mamba model, forming a modular and scalable architecture for efficient sequence modeling~\cite{mamba_architecture}.
